Automatically Debugging AutoML Pipelines using Maro: ML Automated Remediation Oracle (Extended Version)

Machine learning in practice often involves complex pipelines for data cleansing, feature engineering, preprocessing, and prediction. These pipelines are composed of operators, which have to be correctly connected and whose hyperparameters must be correctly configured. Unfortunately, it is quite common for certain combinations of datasets, operators, or hyperparameters to cause failures. Diagnosing and fixing those failures is tedious and error-prone and can seriously derail a data scientist's workflow. This paper describes an approach for automatically debugging an ML pipeline, explaining the failures, and producing a remediation. We implemented our approach, which builds on a combination of AutoML and SMT, in a tool called Maro. Maro works seamlessly with the familiar data science ecosystem including Python, Jupyter notebooks, scikit-learn, and AutoML tools such as Hyperopt. We empirically evaluate our tool and find that for most cases, a single remediation automatically fixes errors, produces no additional faults, and does not significantly impact optimal accuracy nor time to convergence.

==> 7-conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

This paper presents \tool, a tool for automatic debugging of machine learning
pipelines that supports a full, explained round-trip of a remediated pipeline
that is suitable for further AutoML tasks.


% \tool is designed to work in concert with AutoML, which it leverages to
% generate pipeline instances for debugging analysis,
% and with SMT, which it uses to discover constraints that characterize
% succeeding instances.
% \tool supports a full round-trip, as its output is a remediated
% planned pipeline in the same language as its input, suitable for
% further automated search and optimization.

%% We demonstrate the capabilities through an empirical
%% evaluation of the debugging of example planned pipelines with varying
%% degrees of complexity in their faults and necessary remediations.
%% For most cases, our single remediation produces no additional faults and does not significantly impact optimal accuracy.

%Although for this initial work we focus on correctness and remediating faults, our solver-based approach is flexible enough that different types of constraints could be added to the tool. As a simple example, rather than only focusing on the outcome of binary success or failure, future work may also constrain for outcomes such as low performance or undesirable characteristics such as bias. Integrating a MaxSMT solver into \tool would then allow for reasoning about optimization problems as well. Such future work would enable \tool to work even more closely with AutoML optimizers, perhaps improving search performance by reasoning about which sections of the search space are less likely to perform well or contain potential bias.


==> fig_acc_charts.tex <==

\begin{figure}[h]
  \centering
  \includegraphics[width=0.85\columnwidth]{fig_acc_case_a.png}
  \vspace{-3mm}
  \caption{Comparison of original and remediated test set accuracy for case study (a).}
\Description{Comparison of original and remediated test set accuracy for case studies (a).}
\label{fig:acc_a}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.85\columnwidth]{fig_acc_case_b.png}
  \vspace{-3mm}
  \caption{Comparison of original and remediated test set accuracy for case study (b).}
\Description{Comparison of original and remediated test set accuracy for case study (b).}
\label{fig:acc_b}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.85\columnwidth]{fig_acc_case_c.png}
  \vspace{-3mm}
  \caption{Comparison of original and remediated test set accuracy for case study (c).}
\Description{Comparison of original and remediated test set accuracy for case study (c).}
\label{fig:acc_c}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.85\columnwidth]{fig_acc_case_d.png}
  \vspace{-3mm}
  \caption{Comparison of original and remediated test set accuracy for case study (d).}
\Description{Comparison of original and remediated test set accuracy for case study (d).}
\label{fig:acc_d}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.85\columnwidth]{fig_acc_case_e.png}
  \vspace{-3mm}
  \caption{Comparison of original and remediated test set accuracy for case study (e).}
\Description{Comparison of original and remediated test set accuracy for case study (e).}
\label{fig:acc_e}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.85\columnwidth]{fig_acc_case_f.png}
  \vspace{-3mm}
  \caption{Comparison of original and remediated test set accuracy for case study (f).}
\Description{Comparison of original and remediated test set accuracy for case study (f).}
\label{fig:acc_f}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.85\columnwidth]{fig_acc_case_g.png}
  \vspace{-3mm}
  \caption{Comparison of original and remediated test set accuracy for case study (g).}
\Description{Comparison of original and remediated test set accuracy for case study (g).}
\label{fig:acc_g}
\end{figure}


==> fig_accuracy.tex <==
\begin{table}
\centerline{\begin{tabular}{c | c | r | c | r}
Pipeline & Orig.~acc & Orig.~iter & Rem.~acc & Rem.~iter\\
\hline
(a) & 0.7297 & \textbf{203.4} & \textbf{0.7303} & 317.8 (317.8) \\
(b) & 0.7515 & 241.2 & \textbf{0.7624} & 797.8 \textbf{(131.0)} \\
(c) & \textbf{0.7576} & 549.2 & 0.7570 & 561.0 \\
(d) & 0.8333 & 10.2 & 0.8333 & \textbf{4.8} \\
(e) & 1.0000 & 16.0 & 1.0000 & \textbf{12.0} \\
(f) & 0.9750 & 42.4 & \textbf{0.9761} & 310.4 \textbf{(17.2)} \\
(g) & \textbf{0.9756} & 134.6 & 0.9750 & 122.0 \\
(h) & 0.7297 & \textbf{50.8} & \textbf{0.7303} & 181.6 (181.6) \\
(i) & 0.8333 & 17.0 & 0.8333 & \textbf{1.0} \\
(j) & \textbf{0.7273} & 94.8 & 0.7267 & 345.2 \\
(k) & 0.7515 & 382.6 & \textbf{0.7570} & 672.6 \textbf{(5.0)} \\
(l) & 0.7515 & 193.8 & \textbf{0.7564} & 615.6 \textbf{(5.0)} \\
(m) & 0.7091 & 2.0 & 0.7091 & \textbf{1.0} \\
(n) & 0.8333 & 17.0 & 0.8333 & \textbf{1.0} \\
(o) & 0.9667 & 105.4 & \textbf{1.0000} & \textbf{77.8} \textbf{(77.8)} \\
(p) & 0.9772 & \textbf{204.6} & \textbf{0.9783} & 223.4 (223.4) \\
(q) & 0.0778 & 1.0 & 0.0778 & 1.0 \\
(r) & \textbf{0.7212} & 84.8 & 0.7206 & 152.4 \\
(s) & 1.0000 & \textbf{99.0} & 1.0000 & 950.0 \\
(t) & \textbf{0.7739} & 558.0 & 0.7709 & 104.8 \\
\end{tabular}}
\vspace*{2mm}
\caption{\label{tab:accuracy}Average optimal test set accuracy (acc) and iterations (iter) to reach it for original (orig) and remediated (rem). In cases where rem acc is higher, rem iter includes average iterations to match orig acc in parantheses.}
\vspace{-9mm}
\end{table}


==> fig_accuracy_old.tex <==
\begin{table}
\centerline{\begin{tabular}{c | r | r | r | r}
Pipeline & Orig.~acc & Orig.~iter & Rem.~acc & Rem.~iter \\
\hline
(a) & 0.727 & 15  & 0.727 & 9   \\
(b) & 0.733 & 27  & 0.727 & 32  \\
(c) & 0.730 & 39  & 0.742 & 286 \\
(d) & 0.833 & 21  & 0.833 & 3   \\
(e) & 1.000 & 16  & 1.000 & 5   \\
(f) & 0.975 & 39  & 0.981 & 67  \\
(g) & 0.975 & 102 & 0.975 & 69  \\
(h) & 0.727 & 18  & 0.727 & 9   \\
(i) & 0.833 & 17  & 0.833 & 1   \\
(j) & 0.727 & 16  & 0.727 & 1   \\
(k) & 0.736 & 113 & 0.752 & 445  \\
(l) & 0.733 & 129 & 0.745 & 241  \\
(m) & 0.709 & 2   & 0.709 & 1   \\
(n) & 0.833 & 17  & 0.833 & 1   \\
(o) & 1.000 & 77  & 1.000 & 47  \\
(p) & 0.975 & 2   & 0.978 & 128 \\
(q) & 0.078 & 1   & 0.078 & 1   \\
(r) & 0.724 & 10  & 0.724 & 1   \\
(s) & 1.000 & 99  & 0.833 & 74  \\
(t) & 0.776 & 166 & 0.773 & 219 \\
\end{tabular}}
\vspace*{2mm}
\caption{\label{tab:accuracy}Best test set accuracy (acc) and iterations (iter) to reach it for original (orig) and remediated (rem) pipelines.}
\vspace{-9mm}
\end{table}


==> sec_explanation.tex <==
\subsection{Explanation}\label{sec:explanation}

When we built \tool, we wanted the explanations it produces to use
familiar syntax, be concise, and refer only to things that the data
scientist has control over. The latter is taken care of by \tool's
remediation, which takes a black-box approach (no tracing
into operator implementations or into dataset characteristics). That
leaves familiarity and conciseness.  Initially, for conciseness, we
just printed the logic formula that comes back from the SMT solver. But
while this was useful for us to develop our tool, we found that it
looks too different from the original user-written Python code to
expect the general user population to appreciate it.

Therefore, instead, we built a pretty-printer
for pipelines that is optimized for readability and ease of diffing.
Specifically, our pretty-printer introduces intermediate variables for
interesting operator configurations, with a standard naming scheme to
prevent spurious differences. To make sure the pretty-printed code can
be trusted, we created extensive round-trip tests, asserting that the
result of print$+$eval$+$print is the same as the result of a single
print. This was helpful especially for sophisticated cases such as
pretty-printing calls to \python{customize_schema}.

With the
pretty-printing feature in hand, users of \tool can inspect the entire
remediated pipeline, which is often useful in and of itself. But
sometimes users find this format not concise enough, as it makes it
tedious to do the diff against the original planned pipeline in their
mind. So in addition, we implemented the \python{pipeline_diff}
functionality that was demonstrated in
Section~\ref{sec:detailed_example}. It simply pretty-prints both the
original planned pipeline and the remediated pipeline to strings, then
uses an off-the-shelf diffing library on them, and finally renders the
result using Markdown highlighting in a notebook.

